Double Threshold based Optimal Device Selection Scheme for D2D or Sidelink Network

Device-to-device (D2D) or Sidelink aided communication is regarded as one of the most promising technologies to improve the spectral efficiency of the 5G and beyond communication system. However, two main challenges exist: 1) the selection of the optimal number of devices for improving the spectral efficiency, and 2) improving the physical layer security of such a communication system. The optimal device improves the secrecy capacity, and the selection of optimal devices enhances the physical layer security. Therefore, in this paper, we propose a double threshold-based optimal device selection (ODS) scheme for a cooperative wireless network with amplify and forward (AF) protocol in the presence and absence of an eavesdropper to enhance the physical layer security for the D2D network. The proposed scheme is analyzed with different distance cases, device scenarios, and modulation schemes. The bit error rate (BER) performance analysis concludes that a performance gain of more than 4 dB is achieved at the BER of 0:004 for the proposed double threshold-based ODS scheme compared to the existing ODS scheme at a high signal to noise ratio (SNR). Furthermore, the proposed scheme enhances the physical layer security.

==> System_Model.tex <==
\section{SYSTEM MODEL}~\label{sec:System-Model}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
\begin{figure}[!t]
\centering
\includegraphics[width=1.0\linewidth]{D2D3.jpg}
\caption{Cooperative communication system}
\label{fig:fig-1}
\end{figure}

In figure~\ref{fig:fig-1}, the source $S$ transmits the information to the end device $ED$. There are a number of devices which can also assist in the transmission of this information. Generally, these devices are represented as $D_1, D_2, \cdots, D_N$. In order to design and develop robust threshold mechanism  we have considered the presence of an eavesdropper $E$. Passive eavesdropper is considered in this paper, where $E$ is located near to the devices node which are involved in accessing the source information. The communications takes place during two phases. In Phase-$I$, $S$ broadcasts the transmitted signal $x$, that is received by all devices, $E$ and $ED$. The $N$ devices are selected based on input threshold $\gamma_{i}$. The amplified signal is forwarded by the set of $N$ selected devices to the $ED$ in Phase-$II$. Out of these $N$ devices some will be dropped depending upon the output threshold $\gamma_o$. Both these thresholds will be discussed in detail in the relevant section. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%555
\subsection{Phase-$I$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The signal received at $ED$ through the direct link in Phase-$I$ is given as
\begin{equation}~\label{eq-1}
    y_{S,ED} = \sqrt{P_s}h_{S,ED}x + n_{S,ED}, 
\end{equation}
where $P_s$ denotes the average source power of the transmitted signal. The signal received at the device in Phase-$I$ is given as
%
\begin{equation}~\label{eq-2}
    y_{S,D_i} = \sqrt{P_s}h_{S,D_i}x + n_{S,D_i}, \quad i = 1,2,\cdots, 
\end{equation}
%
In equation (\ref{eq-1}) and (\ref{eq-2}) the terms $n_{S,ED}$ and $n_{S,D_i}$ is the complex additive white Gaussian noise with zero-mean and variance $N_0$. Similarly, the channel between source and the end device $h_{S,ED}$ and source to the $i$-th device node $h_{S,D_i}$ is modelled as Rayleigh faded.
\begin{itemize}
\item {\bf Input Threshold, $\gamma_i$:} The input threshold $\gamma_i$ depends on the distance between $S$ and the $i$-th device. The instantaneous SNR of the source to the $i$-th device is given as
%
\begin{equation}~\label{eq-3}
    \gamma_{S,D_i}=\frac{P_s\zeta_i^2}{N_0}, \quad i=1,2,\cdots,
\end{equation}
%
where $\zeta_i^2=|h_{S, D_i}^2|$ is the channel coefficient of the source to the $i$-th device. The $i$-th device will compares the instantaneous SNR as calculated in (\ref{eq-3}) with this input threshold $\gamma_i$. If the instantaneous SNR is above $\gamma_i$, then the device is selected. If the instantaneous SNR of the device is lower than the input threshold the device is not selected. The selection condition of the $i$-th device can be represented as
%
\begin{eqnarray}~\label{eq-4}
\textrm{Device, $D_i$}=\left\{
\begin{matrix}
\gamma_{S, D_i}\geq \gamma_{i} &\textrm{Selected} \\
\gamma_{S, D_i}< \gamma_{i} & \textrm{Not Selected}.
\end{matrix}
\right.
\end{eqnarray}
%
\end{itemize}
%
%%%%%%%%%%%%%%%%555555
\subsection{Phase-$II$}
%%%%%%%%%%%%%%%%%%%%%%%5
\begin{figure*}[!tbh]
\begin{eqnarray}~\label{eq-9}
\setcounter{equation}{9}
\textrm{Selected Transmission Link}=\left\{ 
\begin{matrix}
& \gamma_{S,ED}+\gamma_{D_i, ED}, &\gamma_{S, ED} >\gamma_{o}  ~~\textrm{and}~~\gamma_{S, D_i}>\gamma_{i}, \\
& \gamma_{S, ED}, & \gamma_{S, D_i}<\gamma_{i}\\
& \gamma_{D_i, ED}, & ~~\gamma_{S, ED}<\gamma_{o},\\
& 0, &\gamma_{S, ED}<\gamma_{o}~~ \textrm{and}~~ \gamma_{D_i,ED}<\gamma_{o}\\
\end{matrix}
\right.
\end{eqnarray}
\hline
\end{figure*}
In this phase, the $N$ selected devices employ the amplified and forward (AF) protocol. The amplification factor at the selected $i$-th device is given as~\cite{Laneman-2004}
%
\begin{equation}~\label{eq-5}
\setcounter{equation}{5}
\alpha_{i}=\frac{\sqrt{P_{D_i}}}{\sqrt{P_s\zeta_i^2+N_0}},\quad i=1,2,\cdots,N,
\end{equation}
%
where $P_{D_i}$ is the average power applied by the $i$-th device $D_i$. The received signal at the end device is given as
%
\begin{equation}~\label{eq-6}
y_{D_i, ED} = \alpha_i h_{D_i, ED}y_{s, D_i}+n_{D_i, ED},
\end{equation}
%
where $n_{D_i, ED}$ is the complex additive white Gaussian noise with zero-mean and variance $N_0$ and $h_{D_i,ED}$ is the channel gain between the $i$-th device and the end device and experiences Rayleigh fading. At the end device, we consider two different kind of optimal device selection scheme (ODS). In the first kind the wiretap link between the $i$-th device and the $E$ is considered while in the second kind of the wiretap link is ignored. 
\begin{itemize}
\item {\bf ODS with Eavesdropper:} The optimal device selection scheme (ODS) that consider the wiretap channel, $S$, $E$, $D_i$, and $ED$, the secrecy capacity is maximized as mentioned in (12) in ~\cite{Zou-2013} as 
%
\begin{eqnarray}~\label{eq-7}
    \textrm{ODS} = arg \max_{i \in D_N} \frac{1+\frac{P_S \zeta_1^2\zeta_2^2}{2(\zeta_1^2+\zeta_2^2)\sigma_n^2}}{1+\frac{P_S \zeta_1^2\zeta_3^2}{2(\zeta_1^2+\zeta_3^2)\sigma_n^2}},
\end{eqnarray}
%
where $\zeta_2^2=|h_{D_i, ED}^2|$ and $\zeta_3^2=|h_{D_i, E}^2|$ is the channel coefficient of the $i$-th device to eavesdropper $E$. 

\item{\bf ODS without Eavesdropper:} The ODS based scheme that does not consider the wiretap link, the maximum capacity from the $i$-th device to end device $ED$ is given as (13) in ~\cite{Zou-2013} as
%
\begin{eqnarray}~\label{eq-8}
    \textrm{ODS} = arg \max_{i \in D_N} \frac{\zeta_1^2\zeta_2^2}{\zeta_1^2+\zeta_2^2}.
\end{eqnarray}
%
\item {\bf Output Threshold:} The signal at the end device $ED$ will be weak and the output signal will be degraded if the link between the device $D$ and the end device $ED$ has high fading. The output threshold at the combiner  selects the best device to end device link from the $i$-th device to the end device. The threshold set at the output of the combiner $\gamma_o$ test the effect of selected $i$-th device and the signal from the direct link. Output threshold testing condition is given in (\ref{eq-10}).
\end{itemize}
